AI-Assisted Colonoscopy: Polyp Detection and Segmentation using Foundation Models

In colonoscopy, 80% of the missed polyps could be detected with the help of Deep Learning models. In the search for algorithms capable of addressing this challenge, foundation models emerge as promising candidates. Their zero-shot or few-shot learning capabilities, facilitate generalization to new data or tasks without extensive fine-tuning. A concept that is particularly advantageous in the medical imaging domain, where large annotated datasets for traditional training are scarce. In this context, a comprehensive evaluation of foundation models for polyp segmentation was conducted, assessing both detection and delimitation. For the study, three different colonoscopy datasets have been employed to compare the performance of five different foundation models, DINOv2, YOLO-World, GroundingDINO, SAM and MedSAM, against two benchmark networks, YOLOv8 and Mask R-CNN. Results show that the success of foundation models in polyp characterization is highly dependent on domain specialization. For optimal performance in medical applications, domain-specific models are essential, and generic models require fine-tuning to achieve effective results. Through this specialization, foundation models demonstrated superior performance compared to state-of-the-art detection and segmentation models, with some models even excelling in zero-shot evaluation; outperforming fine-tuned models on unseen data.

==> references.tex <==
% Include here your reference list.

% Use BIBTEX format for reference entries:
@article{missedpolyps,
  author = {Kim, Nam and Jung, Yoon and Jeong, Woo and Yang, Hyo-Joon and Park, Soo-Kyung and Choi, Kyuyong and Park, Dong},
  title = {Miss rate of colorectal neoplastic polyps and risk factors for missed polyps in consecutive colonoscopies},
  journal = {Intestinal Research},
  year = {2017},
  volume = {15},
  number = {3},
  pages = {411},
  doi = {10.5217/ir.2017.15.3.411},
  month = {Jul},
}

@article{dinov2,
title={{DINO}v2: Learning Robust Visual Features without Supervision},
author={Maxime Oquab and Timoth{\'e}e Darcet and Th{\'e}o Moutakanni and Huy V. Vo and Marc Szafraniec and Vasil Khalidov and Pierre Fernandez and Daniel HAZIZA and Francisco Massa and Alaaeldin El-Nouby and Mido Assran and Nicolas Ballas and Wojciech Galuba and Russell Howes and Po-Yao Huang and Shang-Wen Li and Ishan Misra and Michael Rabbat and Vasu Sharma and Gabriel Synnaeve and Hu Xu and Herve Jegou and Julien Mairal and Patrick Labatut and Armand Joulin and Piotr Bojanowski},
journal={Transactions on Machine Learning Research},
issn={2835-8856},
year={2024}
}

@article{miccai,
  author = {Bernal, Jorge and Tajbakhsh, Nima and Sanchez, Francisco and Matuszewski, Bogdan and Chen, Hao and Yu, Lequan and Angermann, Quentin and Romain, Olivier and Rustad, Bjorn and Balasingham, Ilangko and Pogorelov, Konstantin and Choi, Sungbin and Debard, Quentin and Maier-Hein, Lena and Speidel, Stefanie and Stoyanov, Danail and Brandao, Patrick and Córdova, Henry and Sánchez-Montes, Cristina and Histace, Aymeric},
  title = {Comparative Validation of Polyp Detection Methods in Video Colonoscopy: Results From the MICCAI 2015 Endoscopic Vision Challenge},
  journal = {IEEE Transactions on Medical Imaging},
  year = {2017},
  volume = {36},  
  number = {6},   
  pages = {1231-1249},
  doi = {10.1109/TMI.2017.2664042},
  month = {Feb},
}

@inproceedings{sameg,
  author    = {Trinh, Quoc-Huy and Nguyen, Hai-Dang and Tram, Nguyen Ngoc Bao and Jha, Debesh and Bagci, Ulas and Tran, Minh-Triet},
  title     = {SAM-EG: Segment Anything Model with Edge Guidance Framework for Efficient Polyp Segmentation},
  booktitle = {Proceedings of the 35th British Machine Vision Conference (BMVC 2024), Glasgow, UK, November 25-28, 2024},
  publisher = {BMVA},
  year      = {2024},
  url       = {https://papers.bmvc2024.org/0472.pdf},
}

@inproceedings{dino,
title={{DINO}: {DETR} with Improved DeNoising Anchor Boxes for End-to-End Object Detection},
author={Hao Zhang and Feng Li and Shilong Liu and Lei Zhang and Hang Su and Jun Zhu and Lionel Ni and Heung-Yeung Shum},
booktitle={The Eleventh International Conference on Learning Representations },
year={2023}
}

@article{nice,
  author = {Hattori, Santa and Iwatate, Mineo and Sano, Wataru and Hasuike, Noriaki and Kosaka, Hidekazu and Ikumoto, Taro and Kotaka, Masahito and Ichiyanagi, Akihiro and Ebisutani, Chikara and Hisano, Yasuko and Fujimori, Takahiro and Sano, Yasushi},
  title = {Narrow-band imaging observation of colorectal lesions using NICE classification to avoid discarding significant lesions},
  journal = {World J. Gastrointest. Endosc.},
  volume = {6},
  number = {12},
  pages = {600--605},
  month = {Dec.},
  year = {2014},
  doi = {10.4253/wjge.v6.i12.600}
}

@article{CRC,
author = {E. Kuipers and W. Grady and D. Lieberman and T. Seufferlein and J. Sung and P. G. Boelens and J. Cornelis and V. Van Velde and T. Watanabe},
title = {Colorectal cancer},
journal = {Nature Reviews Disease Primers},
volume = {ePub ahead of print},
year = {2015},
month = {Dec.},  
doi = {10.1038/nrdp.2015.65},
}

@misc{acs_colorectal_2025,
  author       = {American Cancer Society},
  title        = {Key Statistics for Colorectal Cancer},
  year         = {2024},
  note         = {Accessed: 2025-03-13},
  howpublished = {\url{https://www.cancer.org/cancer/types/colon-rectal-cancer/about/key-statistics.html}},
  month        = {Dec.}
}

@article{cure,
  author = {W. Atkin and R. Edwards and I. Kralj-Hans and K. Wooldrage and A. Hart and J. Northover and D. Parkin and J. Wardle and S. Duffy and J. Cuzick},
  title = {Once-only flexible sigmoidoscopy screening in prevention of colorectal cancer: A multicentre randomised controlled trial},
  journal = {Lancet}, 
  volume = {375},  
  pages = {1624--1633}, 
  month = {May}, 
  year = {2010}, 
  doi = {10.1016/S0140-6736(10)60551-X}
}

@article{origin,
  author = {Mármol, Inés and Sánchez de Diego, Cristina and Pradilla-Dieste, Alberto and Cerrada, Elena and Rodríguez-Yoldi, Maria},
  year = {2017},
  title = {Colorectal Carcinoma: A General Overview and Future Perspectives in Colorectal Cancer},
  journal = {Int. J. Mol. Sci.},
  volume = {18},
  number = {1},
  pages = {197},
  doi = {10.3390/ijms18010197},
  month = {Jan.},
}

@article{PICCOLO,
  author = {Sanchez-Peralta, L. F. and Pagador, J. B. and Picon, A. and Calderon, A. J. and Polo, F. and Andraka Rueda, N. and Bilbao, R. and Glover, B. and Saratxaga, C. and Sánchez-Margallo, F.},
  year = {2020},
  month = {Dec.},
  title = {PICCOLO White-Light and Narrow-Band Imaging Colonoscopic Dataset: A Performance Comparative of Models and Datasets},
  journal = {Applied Sciences},
  volume = {10},
  number = {12},
  pages = {8501},
  doi = {10.3390/app10238501}
}

@article{Paris,
  author = {Axon, A. and Diebold, M. and Fujino, M. and Fujita, Rikiya and Genta, Robert and Gonvers, Jean-Jacques and Guelrud, Moises and Inoue, H. and Jung, M. and Kashida, Hiroshi and Kudo, S. and Lambert, R. and Lightdale, C. and Nakamura, T. and Neuhaus, H. and Niwa, H. and Ogoshi, K. and Rey, Jean-Francois and Riddell, R. and Yoshida, S.},
  year = {2005},
  month = {Jun.},
  pages = {570--578},
  title = {Update on the Paris Classification of Superficial Neoplastic Lesions in the Digestive Tract},
  volume = {37},
  journal = {Endoscopy},
  doi = {10.1055/s-2005-861352}
}

@article{piccoloproject,
  author = {J. Ortega Morán and A. Azpeitia and L. F. Sanchez-Peralta and L. Bote-Curiel and J. B. Pagador and V. Cabezón and C. Saratxaga and F. Sánchez-Margallo},
  title = {Medical needs related to the endoscopic technology and colonoscopy for colorectal cancer diagnosis},
  journal = {BMC Cancer},
  volume = {21},
  month = {Apr}, 
  year = {2021},
  doi = {10.1186/s12885-021-08190-z},
}

@article{malignantpolyp,
  author = {Bujanda, Luis and Cosme, Angel and Gil, Ines and Arenas-Mirave, Juan},
  year = {2010},
  month = {Jul.},
  title = {Malignant colorectal polyps},
  journal = {World J. Gastroenterol.},
  volume = {16},
  number = {25},
  pages = {3103--3111},
  doi = {10.3748/wjg.v16.i25.3103},
}

@article{SOTA1,
  author = {Sanchez-Peralta, Luisa F. and Bote-Curiel, Luis and Picon, Artzai and Sánchez-Margallo, Francisco and Pagador, J Blas},
  year = {2020},
  month = {Aug},
  pages = {101923},
  title = {Deep learning to find colorectal polyps in colonoscopy: A systematic literature review},
  volume = {108},
  journal = {Artificial Intelligence in Medicine},
  doi = {10.1016/j.artmed.2020.101923},
}

@inproceedings{vggimage,
  author = {Simonyan, Karen and Zisserman, Andrew},
  booktitle = {ICLR},
  crossref = {conf/iclr/2015},
  title = {Very Deep Convolutional Networks for Large-Scale Image Recognition.},
  year = {2015}
}

@INPROCEEDINGS{resnet,
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={2016 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}, 
  title={Deep Residual Learning for Image Recognition}, 
  year={2016},
  pages={770-778},
  doi={10.1109/CVPR.2016.90}
}

@article{dilatedresfcn,
  author = {Y. Guo, J. Bernal, B. Matuszewski},
  title = {Polyp Segmentation with Fully Convolutional Deep Neural Networks—Extended Evaluation Study},
  journal = {J. Imaging},
  vol = {6},
  no = {7},
  pages = {69},
  month = {Jul.},
  year = {2020},
  doi = {10.3390/jimaging6070069},
}

@article{unet,
  author={Weng, Wenlong and Zhu, Xiaoqian},
  title={U-Net: Convolutional Networks for Biomedical Image Segmentation},
  journal={IEEE Access},
  volume={9},
  number={9},
  pages={16591--16603},
  month={Sep},  
  year={2015},
  doi={10.1109/ACCESS.2015.2468207},  
  publisher={IEEE}
}

@article{polypsam++,
author = {Biswas, Risab},
year = {2023},
month = {09},
title = {Polyp-SAM++: Can A Text Guided SAM Perform Better for Polyp Segmentation?},
doi = {10.13140/RG.2.2.35120.53764/2}
}

@INPROCEEDINGS{huang,
  author={Huang, Cheng-Hsien and Xiao, Wei-Ting and Chang, Li-Jen and Tsai, Wei-Ta and Liu, Wei-Min},
  booktitle={2018 IEEE Visual Communications and Image Processing (VCIP)}, 
  title={Automatic tissue segmentation by deep learning: from colorectal polyps in colonoscopy to abdominal organs in CT exam}, 
  year={2018},
  volume={},
  number={},
  pages={1-4},
  keywords={Colonoscopy;Image segmentation;Computed tomography;Feature extraction;Training;Cancer;Colon cancer;CT image organ segmentation;Radiotherapy;Deep learning;Long short term memory network},
  doi={10.1109/VCIP.2018.8698645}}

@article{alamfattah,
author = {Alam, Md and Fattah, Shaikh Anowarul},
year = {2023},
month = {04},
pages = {106945},
title = {{SR-AttNet}: An Interpretable Stretch–Relax Attention based Deep Neural Network for Polyp Segmentation in Colonoscopy Images},
volume = {160},
journal = {Computers in Biology and Medicine},
doi = {10.1016/j.compbiomed.2023.106945}
}

@article{gan,title={Generative adversarial networks},author={Ian J. Goodfellow and Jean Pouget-Abadie and Mehdi Mirza and Bing Xu and David Warde-Farley and Sherjil Ozair and Aaron C. Courville and Y. Bengio},journal={Communications of the ACM},year={2020},volume={63},pages={139 - 144},doi={10.1145/3422622}}


@article{foundationmodels,
author = {Narayan, Avanika and Chami, Ines and Orr, Laurel and R\'{e}, Christopher},
title = {Can Foundation Models Wrangle Your Data?},
year = {2022},
month = {12},
doi = {10.14778/3574245.3574258},
journal = {Proc. VLDB Endow.},
pages = {738–746}
}

@article{SAM,
  title={Segment Anything},
  author={Kirillov, Alexander and Mintun, Eric and Ravi, Nikhila and Mao, Hanzi and Rolland, Chloe and Gustafson, Laura and Xiao, Tete and Whitehead, Spencer and Berg, Alexander C. and Lo, Wan-Yen and Doll{\'a}r, Piotr and Girshick, Ross},
  journal={arXiv:2304.02643},
  year={2023}
}

@article{MedSAM,
  title    = "Segment anything in medical images",
  author   = "Ma, Jun and He, Yuting and Li, Feifei and Han, Lin and You,
              Chenyu and Wang, Bo",
  journal  = "Nature Communications",
  volume   =  15,
  number   =  1,
  pages    = "654",
  month    =  jan,
  year     =  2024
}

@article{maskrcnn,
author = {He, Kaiming and Gkioxari, Georgia and Dollar, Piotr and Girshick, Ross},
year = {2018},
month = {06},
pages = {1-1},
title = {Mask R-CNN},
volume = {PP},
journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
doi = {10.1109/TPAMI.2018.2844175}
}

@inproceedings{yolo,
	location = {Las Vegas, {NV}, {USA}},
	title = {You Only Look Once: Unified, Real-Time Object Detection},
	isbn = {978-1-4673-8851-1},
	doi = {10.1109/CVPR.2016.91},
	shorttitle = {You Only Look Once},
	eventtitle = {2016 {IEEE} Conference on Computer Vision and Pattern Recognition ({CVPR})},
	pages = {779--788},
	booktitle = {2016 {IEEE} Conference on Computer Vision and Pattern Recognition ({CVPR})},
	publisher = {{IEEE}},
	author = {Redmon, Joseph and Divvala, Santosh and Girshick, Ross and Farhadi, Ali},
	urldate = {2025-01-20},
	date = {2016-06},
	year = {2016},
	langid = {english},
	file = {Redmon et al. - 2016 - You Only Look Once Unified, Real-Time Object Dete.pdf:C\:\\Users\\110567\\Zotero\\storage\\T37Y6VU4\\Redmon et al. - 2016 - You Only Look Once Unified, Real-Time Object Dete.pdf:application/pdf},
}

@misc{yolov8,
  author = {YOLOv8},
  title = {YOLOv8: Real-Time Object Detection},
  howpublished = {\url{https://yolov8.com/}},
  note = {Accessed: 2024-06-03}
}

@inproceedings{yoloworld,
  title={YOLO-World: Real-Time Open-Vocabulary Object Detection},
  author={Cheng, Tianheng and Song, Lin and Ge, Yixiao and Liu, Wenyu and Wang, Xinggang and Shan, Ying},
  booktitle={Proc. IEEE Conf. Computer Vision and Pattern Recognition (CVPR)},
  year={2024}
}

@article{groundingdino_paper,
  title={Grounding dino: Marrying dino with grounded pre-training for open-set object detection},
  author={Liu, Shilong and Zeng, Zhaoyang and Ren, Tianhe and Li, Feng and Zhang, Hao and Yang, Jie and Li, Chunyuan and Yang, Jianwei and Su, Hang and Zhu, Jun and others},
  journal={arXiv preprint arXiv:2303.05499},
  year={2023}
}

@inproceedings{bert,
  title={BERT: Pre-training of Deep Bidirectional Transformers for Language Understanding},
  author={Jacob Devlin and Ming-Wei Chang and Kenton Lee and Kristina Toutanova},
  booktitle={North American Chapter of the Association for Computational Linguistics},
  year={2019},
  url={https://api.semanticscholar.org/CorpusID:52967399}
}

@INPROCEEDINGS {conference,
author = { Huix, Joana Pales and Ganeshan, Adithya Raju and Haslum, Johan Fredin and Soderberg, Magnus and Matsoukas, Christos and Smith, Kevin },
booktitle = { 2024 IEEE/CVF Winter Conference on Applications of Computer Vision (WACV) },
title = {{ Are Natural Domain Foundation Models Useful for Medical Image Classification? }},
year = {2024},
month = {01},
pages = {7619-7628},
doi = {10.1109/WACV57701.2024.00746},
publisher = {IEEE Computer Society},
}


@inproceedings{coco,
  author = {Lin, Tsung-Yi and Maire, Michael and Belongie, Serge and Hays, James and Perona, Pietro and Ramanan, Deva and Dollár, Piotr and Zitnick, C.},
  title = {Microsoft COCO: Common Objects in Context},
  booktitle = {Proceedings of the European Conference on Computer Vision (ECCV)},
  year = {2014},
  month = {May}
}

@inproceedings{clip,
  title={Learning Transferable Visual Models From Natural Language Supervision},
  author={Alec Radford and Jong Wook Kim and Chris Hallacy and Aditya Ramesh and Gabriel Goh and Sandhini Agarwal and Girish Sastry and Amanda Askell and Pamela Mishkin and Jack Clark and Gretchen Krueger and Ilya Sutskever},
  booktitle={International Conference on Machine Learning},
  year={2021},
}

@misc{yoloworld_doc,
  author = {{Ultralytics}},
  title = {YOLO-World Models},
  year = {2024},
  url = {https://docs.ultralytics.com/models/yolo-world/},
  note = {Accessed: 2024-06-04}
}

@misc{groundingdino_github,
  author       = {IDEA Research},
  title        = {GroundingDINO: Open-set Object Detector with Language Grounding},
  year         = {2023},
  url          = {https://github.com/IDEA-Research/GroundingDINO},
  note         = {Accessed: 2024-12-20}
}

@article{groundingdino_mmdetection_ft,
  title   = {{MMDetection}: Open MMLab Detection Toolbox and Benchmark},
  author  = {Chen, Kai and Wang, Jiaqi and Pang, Jiangmiao and Cao, Yuhang and
             Xiong, Yu and Li, Xiaoxiao and Sun, Shuyang and Feng, Wansen and
             Liu, Ziwei and Xu, Jiarui and Zhang, Zheng and Cheng, Dazhi and
             Zhu, Chenchen and Cheng, Tianheng and Zhao, Qijie and Li, Buyu and
             Lu, Xin and Zhu, Rui and Wu, Yue and Dai, Jifeng and Wang, Jingdong
             and Shi, Jianping and Ouyang, Wanli and Loy, Chen Change and Lin, Dahua},
  journal= {arXiv preprint arXiv:1906.07155},
  year={2019}
}

@misc{yolov8_doc,
  title = {Ultralytics YOLOv8 Documentation},
  author = {Glenn Jocher and Ayush Chaurasia and Jing Qiu},
  year = {2024},
  howpublished = {\url{https://docs.ultralytics.com/models/yolov8/}},
  note = {Accessed: 2024-06-09}
}


@InProceedings{polypsegm-ash,
author="Tudela, Yael
and Garc{\'i}a-Rodr{\'i}guez, Ana
and Fern{\'a}ndez-Esparrach, Gl{\'o}ria
and Bernal, Jorge",
editor="Wesarg, Stefan
and Puyol Ant{\'o}n, Esther
and Baxter, John S. H.
and Erdt, Marius
and Drechsler, Klaus
and Oyarzun Laura, Cristina
and Freiman, Moti
and Chen, Yufei
and Rekik, Islem
and Eagleson, Roy
and Feragen, Aasa
and King, Andrew P.
and Cheplygina, Veronika
and Ganz-Benjaminsen, Melani
and Ferrante, Enzo
and Glocker, Ben
and Moyer, Daniel
and Petersen, Eikel",
title="Towards Fine-Grained Polyp Segmentation and Classification",
booktitle="Clinical Image-Based Procedures,  Fairness of AI in Medical Imaging, and Ethical and Philosophical Issues in Medical Imaging",
year="2023",
publisher="Springer Nature Switzerland",
address="Cham",
pages="32--42",
abstract="Colorectal cancer is one of the main causes of cancer death worldwide. Colonoscopy is the gold standard screening tool as it allows lesion detection and removal during the same procedure. During the last decades, several efforts have been made to develop CAD systems to assist clinicians in lesion detection and classification. Regarding the latter, and in order to be used in the exploration room as part of resect and discard or leave-in-situ strategies, these systems must identify correctly all different lesion types. This is a challenging task, as the data used to train these systems presents great inter-class similarity, high class imbalance, and low representation of clinically relevant histology classes such as serrated sessile adenomas.",
isbn="978-3-031-45249-9"
}

@article{sunseg,
author = {Misawa, Masashi and Kudo, shin-ei and Mori, Yuichi and Hotta, Kinichi and Ohtsuka, Kazuo and Matsuda, Takahisa and Saito, Shoichi and Kudo, Toyoki and Baba, Toshiyuki and Ishida, Fumio and Itoh, Hayato and Oda, Masahiro and Mori, Kensaku},
year = {2020},
month = {07},
pages = {},
title = {Development of a computer-aided detection system for colonoscopy and a publicly accessible large colonoscopy video database (with video)},
volume = {93},
journal = {Gastrointestinal Endoscopy},
doi = {10.1016/j.gie.2020.07.060}
}


@misc{medsamgithub,
  author       = {Bo Wang Lab},
  title        = {MedSAM: Segment Anything Model for Medical Images},
  year         = {2024},
  howpublished = {\url{https://github.com/bowang-lab/MedSAM}},
  note         = {Accessed: 2024-11-17}
}

@article{ccstats,
author = {Siegel, Rebecca and Wagle, Nikita Sandeep and Cercek, Andrea and Smith, Robert and Jemal, Ahmedin},
year = {2023},
month = {03},
pages = {},
title = {Colorectal cancer statistics, 2023},
volume = {73},
journal = {CA: A Cancer Journal for Clinicians},
doi = {10.3322/caac.21772}
}

@misc{chen,
      title={{3D TransUNet}: Advancing Medical Image Segmentation through Vision Transformers}, 
      author={Jieneng Chen and Jieru Mei and Xianhang Li and Yongyi Lu and Qihang Yu and Qingyue Wei and Xiangde Luo and Yutong Xie and Ehsan Adeli and Yan Wang and Matthew Lungren and Lei Xing and Le Lu and Alan Yuille and Yuyin Zhou},
      year={2023},
      eprint={2310.07781},
      archivePrefix={arXiv},
      primaryClass={cs.CV},
      url={https://arxiv.org/abs/2310.07781}, 
}

@article{urban2018,
author = {Urban, Gregor and Tripathi, Priyam and Alkayali, Talal and Mittal, Mohit and Jalali, Farid and Karnes, William and Baldi, Pierre},
year = {2018},
month = {06},
pages = {},
title = {Deep Learning Localizes and Identifies Polyps in Real Time With 96\% Accuracy in Screening Colonoscopy},
volume = {155},
journal = {Gastroenterology},
doi = {10.1053/j.gastro.2018.06.037}
}

@article{chenbaldi,
author = {Chen, Siwei and Urban, Gregor and Baldi, Pierre},
year = {2022},
month = {04},
pages = {121},
title = {Weakly Supervised Polyp Segmentation in Colonoscopy Images Using Deep Neural Networks},
volume = {8},
journal = {Journal of Imaging},
doi = {10.3390/jimaging8050121}
}

==> tables/tab1_old.tex <==
\begin{table}[tpb!]  %* for the two columns
\centering
\caption{Detection Performance Comparison}
\label{detection_table}
\setlength{\tabcolsep}{3pt}
%\resizebox{\textwidth}{!}{ % resize to fit textwidth
\resizebox{\columnwidth}{!}{ % resize to fit textwidth
\begin{tabular}{lccccccc}
\toprule
%\multirow{2}{*}{MODEL} & \multirow{2}{*}{FT} & \multicolumn{2}{|c|}{PICCOLO} & \multicolumn{2}{|c|}{PolypSegm-ASH} & \multicolumn{2}{|c|}{SUN-SEG} \\ \cline{3-8} 
\multirow{2}[3]{*}{MODEL} & \multirow{2}[3]{*}{FT} & \multicolumn{2}{c}{PICCOLO} & \multicolumn{2}{c}{PolypSegm-ASH} & \multicolumn{2}{c}{SUN-SEG} \\
%\cline{3-8} 
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}

                       &                     & AP & AR                       & AP & AR                              & AP & AR                       \\
\midrule
Yolov8                 & \checkmark          & 0.529 & 0.587                      & 0.588 & 0.655                             & 0.471 & 0.494                      \\ 
YOLOWorld             &                     & 0.081 & 0.159                      & 0.055 & 0.226                             & $6.7 \mathrm{e}{-5} \approx 0$ & 0.006                      \\ 
YOLOWorld             & \checkmark          & 0.435 & 0.495                      & 0.613 & 0.681                             & 0.497 & 0.524                      \\ 
M R-CNN R50   & \checkmark          & 0.571 & 0.614                      & 0.705 & 0.761                             & 0.472 & 0.507                      \\ 
M R-CNN DINOv2      & \checkmark          & 0.438 & 0.486                      & 0.348 & 0.396                             & 0.311 & 0.352                      \\ 
GDINO         &                     & 0.133 & 0.520                      & 0.072 & 0.369                             & 0.002 & 0.086                      \\ 
GDINO         & \checkmark       & \textbf{0.722} & \textbf{0.805}                     & \textbf{0.794} & \textbf{0.846}                             & \textbf{0.514} & \textbf{0.547}\\
\bottomrule
\end{tabular}
} % end resizebox
\end{table}

==> tables/tab1_uxue.tex <==
\begin{table*}
\centering
\caption{DETECTION PERFORMANCE COMPARISON}
\label{detection_table}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{|p{90pt}|p{20pt}|p{30pt}|p{30pt}|p{30pt}|p{30pt}|p{30pt}|p{30pt}|}
\hline
\multirow{2}{*}{MODEL} & \multirow{2}{*}{FT} & \multicolumn{2}{|c|}{PICCOLO} & \multicolumn{2}{|c|}{PolypSegm-ASH} & \multicolumn{2}{|c|}{SUN-SEG} \\ \cline{3-8} 
                       &                     & AP & AR                       & AP & AR                              & AP & AR                       \\ \hline
Yolov8                 & \checkmark          & 0.529 & 0.587                      & 0.588 & 0.655                             & 0.471 & 0.494                      \\ 
YOLOWorld             &                     & 0.081 & 0.159                      & 0.055 & 0.226                             & \(6.7 \mathrm{e}{-5}\) & 0.006                      \\ 
YOLOWorld             & \checkmark          & 0.435 & 0.495                      & 0.613 & 0.681                             & 0.497 & 0.524                      \\ 
Mask R-CNN ResNet 50   & \checkmark          & 0.571 & 0.614                      & 0.705 & 0.761                             & 0.472 & 0.507                      \\ 
Mask R-CNN DINOv2      & \checkmark          & 0.438 & 0.486                      & 0.348 & 0.396                             & 0.311 & 0.352                      \\ 
GroundingDINO         &                     & 0.133 & 0.520                      & 0.072 & 0.369                             & 0.002 & 0.086                      \\ 
GroundingDINO         & \checkmark       & \textbf{0.722} & \textbf{0.805}                     & \textbf{0.794} & \textbf{0.846}                             & \textbf{0.514} & \textbf{0.547}                      \\ \hline
\end{tabular}
\end{table*}

==> tables/tab2_2col.tex <==
\begin{table*}[htpb!]  %* for the two columns
\centering
\caption{SEGMENTATION PERFORMANCE COMPARISON\alertAAG{why not lowercase?}}
\label{segmentation_table}
\setlength{\tabcolsep}{3pt}
%\resizebox{\textwidth}{!}{ % resize to fit textwidth
%\begin{tabular}{|p{80pt}|p{80pt}|p{20pt}|p{20pt}|p{60pt}|p{60pt}|p{60pt}|}
\begin{tabular}{llccccc}
%\hline
\toprule
%\multicolumn{2}{c}{MODEL} & \multicolumn{2}{c}{FT} & \multirow{2}6]{*}{PICCOLO} & \multirow{2}{*}{PolypSegm-ASH} & \multirow{2}{*}{SUN-SEG} \\ 
\multicolumn{2}{c}{MODEL} & \multicolumn{2}{c}{FT} & & & \\ 

%\cline{1-4} 
\cmidrule(lr){1-2} \cmidrule(lr){3-4}
%Det & Seg & Det & Seg &  &  & \\ 
Det & Seg & Det & Seg & PICCOLO & PolypSegm-ASH & SUN-SEG \\ 

\midrule
Yolov8              & SAM & \checkmark & & 0.628 & 0.701 & 0.727 \\
Yolov8              & MedSAM & \checkmark &  & 0.667 & 0.762 & 0.752 \\ 
YOLOWorld          & SAM &  & & 0.175 & 0.163 & 0.351 \\
YOLOWorld          & MedSAM & & & 0.187 & 0.193 & 0.352 \\ 
YOLOWorld          & SAM & \checkmark & & 0.555 & 0.703 & 0.708 \\
YOLOWorld          & MedSAM & \checkmark & & 0.584 & 0.747 & 0.769 \\ 
Mask R-CNN Resnet50 & Mask R-CNN Resnet50 & \checkmark & \checkmark & 0.681 & 0.829 & 0.764 \\
Mask R-CNN Resnet50 & SAM & \checkmark & & 0.655 & 0.754 & 0.717 \\
Mask R-CNN Resnet50 & MedSAM & \checkmark & & 0.687 & 0.835 &  0.763\\ 
Mask R-CNN DINOv2  & Mask R-CNN DINOv2  & \checkmark & \checkmark & 0.632 &  0.578 & 0.722 \\
Mask R-CNN DINOv2  & SAM & \checkmark & & 0.649 & 0.623 & 0.701 \\
Mask R-CNN DINOv2  & MedSAM & \checkmark & & 0.648 & 0.656 & 0.744 \\ 
GroundingDINO      & SAM &  & & 0.088 & 0.146 & 0.02 \\
GroundingDINO      & MedSAM &  & & 0.239 & 0.178 & 0.02 \\
GroundingDINO      & SAM & \checkmark & & 0.703 & 0.813 & 0.749 \\
GroundingDINO      & MedSAM & \checkmark & & \textbf{0.789} & \textbf{0.885} & \textbf{0.799} \\
\bottomrule
\end{tabular}
%} % end resizebox
\end{table*}


==> tables/tab2_baseline.tex <==
\begin{table}[tpb!]  %* for the two columns
\centering
\caption{\colrev{Segmentation Performance (mIoU) for baseline (top) and foundation model-based methods (bottom). FT=Fine-Tuned.}}
\label{segmentation_table}
\setlength{\tabcolsep}{3pt}
%\resizebox{\textwidth}{!}{ % resize to fit textwidth
\resizebox{\columnwidth}{!}{ % resize to fit textwidth
%\begin{tabular}{|p{80pt}|p{80pt}|p{20pt}|p{20pt}|p{60pt}|p{60pt}|p{60pt}|}
\begin{tabular}{llccc}
%\hline
\toprule
%BASEILNE Det. model & Seg. model & PICCOLO & PolypSegm-ASH & SUN-SEG \\ 
\multirow{2}{*}{Det. model} & \multirow{2}{*}{Seg. model} & \multirow{2}{*}{PICCOLO} & \multirow{2}[-3]{*}{PolypSegm} & \multirow{2}{*}{SUN-SEG} \\
& & & -ASH & \\

% tab1
%\multirow{2}[3]{*}{MODEL} & \multirow{2}[3]{*}{FT} & \multicolumn{2}{c}{PICCOLO} & \multicolumn{2}{c}{PolypSegm-ASH} & \multicolumn{2}{c}{SUN-SEG} \\
%\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}

\midrule
MR-CNN R50 FT & MR-CNN R50 FT & 0.681 & 0.829 & 0.764 \\
\midrule
MR-CNN R50 FT & SAM & 0.655 & 0.754 & 0.717 \\
MR-CNN R50 FT & MedSAM &  0.687 & 0.835 &  0.763\\ 
MR-CNN DINOv2 FT & MR-CNN DINOv2 FT & 0.632 &  0.578 & 0.722 \\
MR-CNN DINOv2 FT & SAM & 0.649 & 0.623 & 0.701 \\
MR-CNN DINOv2 FT & MedSAM & 0.648 & 0.656 & 0.744 \\ 
Yolov8 FT          & SAM & 0.628 & 0.701 & 0.727 \\
Yolov8 FT          & MedSAM & 0.667 & 0.762 & 0.752 \\ 
YOLOWorld          & SAM &  0.175 & 0.163 & 0.351 \\
YOLOWorld          & MedSAM & 0.187 & 0.193 & 0.352 \\ 
YOLOWorld FT       & SAM & 0.555 & 0.703 & 0.708 \\
YOLOWorld FT       & MedSAM & 0.584 & 0.747 & 0.769 \\ 
GDINO      & SAM & 0.088 & 0.146 & 0.02 \\
GDINO      & MedSAM & 0.239 & 0.178 & 0.02 \\
GDINO FT   & SAM & 0.703 & 0.813 & 0.749 \\
GDINO FT   & MedSAM  & \textbf{0.789} & \textbf{0.885} & \textbf{0.799} \\
\bottomrule
\end{tabular}
} % end resizebox
\end{table}


==> tables/tab2_old.tex <==
\begin{table}[tpb!]  %* for the two columns
\centering
\caption{Segmentation Performance: mIoU. FT=Fine-Tuned.}
\label{segmentation_table}
\setlength{\tabcolsep}{3pt}
%\resizebox{\textwidth}{!}{ % resize to fit textwidth
\resizebox{\columnwidth}{!}{ % resize to fit textwidth
%\begin{tabular}{|p{80pt}|p{80pt}|p{20pt}|p{20pt}|p{60pt}|p{60pt}|p{60pt}|}
\begin{tabular}{llccc}
%\hline
\toprule
%\multicolumn{2}{c}{MODEL} & \multicolumn{2}{c}{FT} & \multirow{2}6]{*}{PICCOLO} & \multirow{2}{*}{PolypSegm-ASH} & \multirow{2}{*}{SUN-SEG} \\ 
%\multicolumn{2}{c}{MODEL} & & &\\ 
%\cmidrule(lr){1-2}
%Det & Seg & Det & Seg &  &  & \\ 
Det. model & Seg. model & PICCOLO & PolypSegm-ASH & SUN-SEG \\ 
\midrule
Yolov8 FT          & SAM & 0.628 & 0.701 & 0.727 \\
Yolov8 FT          & MedSAM & 0.667 & 0.762 & 0.752 \\ 
YOLOWorld          & SAM &  0.175 & 0.163 & 0.351 \\
YOLOWorld          & MedSAM & 0.187 & 0.193 & 0.352 \\ 
YOLOWorld FT       & SAM & 0.555 & 0.703 & 0.708 \\
YOLOWorld FT       & MedSAM & 0.584 & 0.747 & 0.769 \\ 
M R-CNN R50 FT & M R-CNN R50 FT & 0.681 & 0.829 & 0.764 \\
M R-CNN R50 FT & SAM & 0.655 & 0.754 & 0.717 \\
M R-CNN R50 FT & MedSAM &  0.687 & 0.835 &  0.763\\ 
M R-CNN DINOv2 FT & M R-CNN DINOv2 FT & 0.632 &  0.578 & 0.722 \\
M R-CNN DINOv2 FT & SAM & 0.649 & 0.623 & 0.701 \\
M R-CNN DINOv2 FT & MedSAM & 0.648 & 0.656 & 0.744 \\ 
GDINO      & SAM & 0.088 & 0.146 & 0.02 \\
GDINO      & MedSAM & 0.239 & 0.178 & 0.02 \\
GDINO FT   & SAM & 0.703 & 0.813 & 0.749 \\
GDINO FT   & MedSAM  & \textbf{0.789} & \textbf{0.885} & \textbf{0.799} \\
\bottomrule
\end{tabular}
} % end resizebox
\end{table}


==> tables/tab2_uxue.tex <==
\begin{table*}
\centering
\caption{SEGMENTATION PERFORMANCE COMPARISON}
\label{segmentation_table}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{|p{80pt}|p{80pt}|p{20pt}|p{20pt}|p{60pt}|p{60pt}|p{60pt}|}
\hline
\multicolumn{2}{|c|}{MODEL}      & \multicolumn{2}{|c|}{FT}            & \multirow{2}{*}{PICCOLO} & \multirow{2}{*}{PolypSegm-ASH} & \multirow{2}{*}{SUN-SEG} \\ \cline{1-4} 
Det & Seg               & Det & Seg                      &                         &                              &                         \\ \hline
Yolov8              & SAM & \checkmark & & 0.628 & 0.701 & 0.727 \\
Yolov8              & MedSAM & \checkmark &  & 0.667 & 0.762 & 0.752 \\ 
YOLOWorld          & SAM &  & & 0.175 & 0.163 & 0.351 \\
YOLOWorld          & MedSAM & & & 0.187 & 0.193 & 0.352 \\ 
YOLOWorld          & SAM & \checkmark & & 0.555 & 0.703 & 0.708 \\
YOLOWorld          & MedSAM & \checkmark & & 0.584 & 0.747 & 0.769 \\ 
Mask R-CNN Resnet 50 & Mask R-CNN Resnet 50 & \checkmark & \checkmark & 0.681 & 0.829 & 0.764 \\
Mask R-CNN Resnet 50 & SAM & \checkmark & & 0.655 & 0.754 & 0.717 \\
Mask R-CNN Resnet 50 & MedSAM & \checkmark & & 0.687 & 0.835 &  0.763\\ 
Mask R-CNN DINOv2  & Mask R-CNN DINOv2  & \checkmark & \checkmark & 0.632 &  0.578 & 0.722 \\
Mask R-CNN DINOv2  & SAM & \checkmark & & 0.649 & 0.623 & 0.701 \\
Mask R-CNN DINOv2  & MedSAM & \checkmark & & 0.648 & 0.656 & 0.744 \\ 
GroundingDINO      & SAM &  & & 0.088 & 0.146 & 0.02 \\
GroundingDINO      & MedSAM &  & & 0.239 & 0.178 & 0.02 \\
GroundingDINO      & SAM & \checkmark & & 0.703 & 0.813 & 0.749 \\
GroundingDINO      & MedSAM & \checkmark & & \textbf{0.789} & \textbf{0.885} & \textbf{0.799} \\\hline
\end{tabular}
\end{table*}


==> tables/tab3_uxue.tex <==
\begin{table*}
\centering
\caption{DETECTION CONDITIONAL EVALUATION}
\label{conditional_eval_table}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{|p{80pt}|p{10pt}|p{15pt}|p{15pt}|p{15pt}|p{15pt}|p{15pt}|p{15pt}|p{15pt}|p{15pt}|p{15pt}|p{15pt}|p{15pt}|p{15pt}|p{15pt}|p{15pt}|p{15pt}|p{15pt}|p{15pt}|p{15pt}|p{15pt}|p{15pt}|}
\hline
\multirow{3}{*}{MODEL} & \multirow{3}{*}{FT} & \multicolumn{4}{|c|}{Light Type} & \multicolumn{6}{|c|}{NICE Type} & \multicolumn{4}{|c|}{Polyp Size} & \multicolumn{6}{|c|}{Paris Classification} \\ \cline{3-22} 
                       &                     & \multicolumn{2}{|c|}{WL} & \multicolumn{2}{|c|}{NBI} & \multicolumn{2}{|c|}{1} & \multicolumn{2}{|c|}{2} & \multicolumn{2}{|c|}{3} & \multicolumn{2}{|c|}{Diminutive} & \multicolumn{2}{|c|}{Small} & \multicolumn{2}{|c|}{Protruded} & \multicolumn{2}{|c|}{Flat Elevated} & \multicolumn{2}{|c|}{Flat} \\ \cline{3-22} 
                       &                     & AP & AR & AP & AR & AP & AR & AP & AR & AP & AR & AP & AR & AP & AR & AP & AR& AP & AR& AP & AR\\ \hline
Yolov8                 & \checkmark          &  0.51     &   0.56    &       0.55     &  0.63  &   0.44   &   0.47    &  0.66     &  0.73     &   0.52    &   0.59 &    0.50   &    0.54   &  0.65     & 0.76 &   0.75    &   0.80    &  0.59     &  0.64     &  0.15     &  0.21   \\ 
YOLOWorld           &   &    0.08                 &   0.20    &   0.07    &         0.10    &    0.01    & 0.04      & 0.08      &  0.08     &  0.15           &  0.32     &   0.06    &  0.08     & 0.00  &  0.00     &  0.11   & 0.16 &   0.00    &   0.00    &      0.00    &   0.00 \\ 
YOLOWorld             & \checkmark          &  0.42     & 0.45      &    0.47   &  0.56     &  0.29     &    0.32   &   0.59    &   0.65    &  0.48     &   0.55    &   0.37    &   0.41    &   0.63    & 0.67 &    0.71   &    0.73   &    0.43   &    0.53   &   0.00    &  0.01    \\ 
Mask R-CNN Resnet 50   & \checkmark          &  0.50     &   0.54    &  0.67     &   0.72    &   0.40    &    0.43   &   0.68    &   0.73    &   0.66    &   0.71    &   0.49    &  0.52     &    0.63   &     0.70    &   0.71    &   0.75    &   0.66    & 0.70  & 0.05   &  0.09   \\ 
Mask R-CNN DINOv2      & \checkmark          &  0.41     &  0.44     &  0.49     &  0.55     &   0.34    &  0.36     &    0.57   &   0.62    &  0.45     &  0.51     &   0.41    &   0.44    &    0.55   & 0.60 &  0.60     &  0.63     &   0.51    &   0.57   &  0.12     &   0.13  \\ 
GroundingDINO         &                     &   0.11    &    0.48   &   0.17    &  0.57     &   0.06    &    0.33   &    0.06   &   0.34    &   0.31    &   0.83    &   0.07    &    0.36   &    0.03   & 0.21  &   0.12    &   0.47    &  0.08     &   0.42    &    0.00   & 0.04   \\ 
GroundingDINO         & \checkmark          &   \textbf{0.69}    &   \textbf{0.78}    &  \textbf{0.76}     &  \textbf{0.84}     &     \textbf{0.58}  &  \textbf{0.69}     &    \textbf{0.74}   &    \textbf{0.80}   &   \textbf{0.85}    &   \textbf{0.91}    &    \textbf{0.62}   &    \textbf{0.72}   &   \textbf{0.79}    & \textbf{0.83}  & \textbf{0.83}      &   \textbf{0.86}    &  \textbf{0.67}     &  \textbf{0.76}     &  \textbf{0.33}     & \textbf{0.54}   \\ \hline
\end{tabular}
\end{table*}

